Adapting LLaMA Decoder to Vision Transformer

This work examines whether decoder-only Transformers such as LLaMA, which were originally designed for large language models (LLMs), can be adapted to the computer vision field. We first "LLaMAfy" a standard ViT step-by-step to align with LLaMA's architecture, and find that directly applying a causal mask to the self-attention brings an attention collapse issue, resulting in the failure to the network training. We suggest to reposition the class token behind the image tokens with a post-sequence class token technique to overcome this challenge, enabling causal self-attention to efficiently capture the entire image's information. Additionally, we develop a soft mask strategy that gradually introduces a causal mask to the self-attention at the onset of training to facilitate the optimization behavior. The tailored model, dubbed as image LLaMA (iLLaMA), is akin to LLaMA in architecture and enables direct supervised learning. Its causal self-attention boosts computational efficiency and learns complex representation by elevating attention map ranks. iLLaMA rivals the performance with its encoder-only counterparts, achieving 75.1% ImageNet top-1 accuracy with only 5.7M parameters. Scaling the model to $\sim$310M and pre-training on ImageNet-21K further enhances the accuracy to 86.0%. Extensive experiments demonstrate iLLaMA's reliable properties: shape-texture bias, calibration, quantization compatibility, ADE20K segmentation and CIFAR transfer learning. We hope our study can kindle fresh views to visual architectures in the wave of LLMs and inspire the development of unified multimodal models. Pre-trained models and codes are available https://github.com/techmonsterwang/iLLaMA.

==> figText/fig_llama_bar.tex <==
\begin{wrapfigure}{r}{0.62\textwidth}
\vspace{-1.1em}
\centering
\small
\includegraphics[width=0.99\linewidth]{figure/llama_bar.pdf}
\caption{Rank analysis of the attention map in head 1, layer 1 of the pretrained ViT-T and iLLaMA-T with $N=197$. Difference between them is about 53. The detailed accuracy on each modification can be found in the appendix.}
\label{fig:rank_analysis}
\vspace{-0.99em}
\end{wrapfigure}

==> figText/fig_train_loss_tiny.tex <==
\begin{figure}[h]\centering
\includegraphics[width=0.99\linewidth]{figure/train_loss_tiny.pdf}\\
\vspace{-.7em}
\caption{\textbf{Training curves for iLLaMA-T/16 w/ and w/o soft mask.} 
When soft mask ends, the model experiences a clear rise and then fall in training loss, and eventually reach a lower test loss.}
\label{fig:train_loss_tiny}
\vspace{-.9em}
\end{figure}

==> figText/tab_hyper_large.tex <==
\begin{table*}[b]

\tablestyle{8.0pt}{1.07}
\footnotesize
% \vspace{-3em}
\begin{tabular}{@{\hskip 1ex}l|c@{\hskip 1ex}cc@{\hskip 1ex}c} \\
% \vspace{-8em}
Training Setting & iLLaMA-L & iLLaMA-L & iLLaMA-L \\
& IN-1K training & IN-21K pre-training & IN-1K fine-tuning \\
\shline
\textit{Initialization:} & \\
weight init & trunc. normal (0.2)  \\
\hline \\ [-2ex]
\textit{Training recipe:} & \\
optimizer & AdamW \\
optimizer momentum & $\beta_1, \beta_2{=}0.9, 0.999$  \\
\hline \\ [-2ex]
\textit{Learning hyper-parameters:} & \\
base learning rate & 1e-4  \\
learning rate schedule & cosine decay  \\
weight decay & 0.3  \\
batch size & 4096  \\
training epochs & 300  \\
warmup epochs & 30  \\
warmup schedule & linear  \\
gradient clip & None  \\
exp. mov. avg. (EMA) & 0.9999 \\
layer scale & 1e-6  \\
\hline \\ [-2ex]
\textit{Dropout:} & \\
dropout rate & 0.0 \\
stochastic depth rate & 0.2 \\
\hline \\ [-2ex]
\textit{Data augmentation:} & \\
input resolution & $224^2$ \\
randAugment & (9, 0.5)  \\
random erasing & 0.25  \\
label smoothing & 0.1  \\
mixup  & 0.95  \\
cutmix & 1.0  \\
\hline \\ [-2ex]
\textit{Soft mask:} & \\
soft mask schedule & constant \\
cutoff epochs & 50 \\


\end{tabular}
\caption{\textbf{Our (pre-)training recipe for iLLaMa large model on ImageNet-1K/21K, and fine-tuning recipe on ImageNet-1K.}, adapted from~\cite{liu2023dropout} and~\cite{he2022masked}.}
\vspace{6em}
\label{tab:setup_modified}
\end{table*}

==> figText/tab_hyper_softmask.tex <==
\begin{table}[h]
\centering
\centering
\small
\addtolength{\tabcolsep}{1pt}
\def\arraystretch{1.15}% 
\begin{tabular}{llc}
% \toprule
\multirow{2}{*}{method}      & \multirow{2}{*}{configuration} & model size         \\ 
                           &                                & tiny/small/base    \\ 
\shline
\multirow{2}{*}{data augment.} & mixup                          & 0.1/xx/0.95      \\ 
                           & cutmix                         & 0.1/xx/1.0      \\ 
\hline
\multirow{2}{*}{soft mask}  & schedule      & constant/constant/linear \\ 
                           & cutoff epochs   & 50/xx/25       \\ 
                           & lr warmup   & 5/xx/50       \\ 
% \bottomrule

\end{tabular}
% \vspace{-.5em}
\caption{\textbf{Hyper-parameters on data augmentation and soft mask} for iLLaMA on ImageNet-1K. See Table~\ref{tab:setup_modified} for more details.}

\label{tab:setup_softmask}
\end{table}

==> figText/tab_large.tex <==
\begin{table}[t]
\tablestyle{4pt}{1.17}
\begin{tabular}{lcc}
model & ImageNet-1K trained & ImageNet-21K pre-trained \\
\shline
ViT-L & 82.6$^*$ & 85.2$^\dagger$ \\
\gr iLLaMA-L & \hlr{P-6/P-7/P-8} & \hlr{eval-3} \\ 
\end{tabular}
% \vspace{-.4em}
\caption{\textbf{Comparing large scale ViT and iLLaMA.} Literature baselines: $*$ \cite{liu2022convnet}, $\dagger$ \cite{dosovitskiy2020image}.
}
\label{tab:abl_large} 
% \vspace{-.5em}
\end{table}


% experiment_id
% 112, 113
% 

==> sec/0_Abstract.tex <==
\begin{abstract}
This work examines whether decoder-only Transformers such as LLaMA, which were originally designed for large language models (LLMs), can be adapted to the computer vision field. 
We first "LLaMAfy" a standard ViT step-by-step to align with LLaMA's architecture, and find that directly applying a causal mask to the self-attention brings an attention collapse issue, resulting in the failure to the network training. 
We suggest to reposition the class token behind the image tokens with a \textit{post-sequence class token} technique to overcome this challenge, enabling causal self-attention to efficiently capture the entire image's information. 
Additionally, we develop a \textit{soft mask} strategy that gradually introduces a causal mask to the self-attention at the onset of training to facilitate the optimization behavior. 
The tailored model, dubbed as \textit{image LLaMA (iLLaMA)}, is akin to LLaMA in architecture and enables direct supervised learning. 
Its causal self-attention boosts computational efficiency and learns complex representation by elevating attention map ranks.
iLLaMA rivals the performance with its encoder-only counterparts, achieving 75.1\% ImageNet top-1 accuracy with only 5.7M parameters. 
Scaling the model to $\sim$310M and pre-training on ImageNet-21K further enhances the accuracy to 86.0\%. 
Extensive experiments demonstrate iLLaMA's reliable properties: shape-texture bias, calibration, quantization compatibility, ADE20K segmentation and CIFAR transfer learning. 
We hope our study can kindle fresh views to visual architectures in the wave of LLMs and inspire the development of unified multimodal models. 




















% Decoder-only Transformers are favored in the context of large language models (LLMs) owing to the exceptional linguistic capabilities exhibited by their pre-trained models. Meanwhile, the domination in visual applications is primarily held by models such as ViT, which are encoder-only Transformer, calling for an architectural alignment. In this paper, we introduce \textit{\underline{D}ecoder-\underline{o}nly V\underline{i}sion \underline{T}ransformer (DoiT)}. We empirically demonstrate that through only \textit{supervised training}, a \textit{non-autoregressive decoder-only} architecture can surprisingly also be used as an image classifier. In the spirit of aligning with the LLaMa decoder, we gradually adjusted components to suit our DoiT. In our exploration, we suggest positioning the [CLS] token at the end of the image patch sequences, instead of at the beginning as in ViT, to enable the causal self-attention module to capture information from each image patch. We show that such decoder-only backbone can achieve comparable performance to the encoder-only ViT in ImageNet classification tasks. We hope DoiT can bring fresh prospects for the component-level alignment of language and vision architectures. 


% S2-BNN 版本
% Decoder-only Transformers are favored in the context of large language models (LLMs) owing to the exceptional linguistic capabilities exhibited by their pre-trained models. Meanwhile, the domination in visual applications is primarily held by models such as ViT, which are encoder-only Transformer, calling for an architectural alignment. In this paper, we focus on this architectural gap by gradually aligning components in the LLaMa decoder to the ViT encoder. 
% We find that xxx do not converge. and found the reason. 
% Instead, we suggest positioning the [CLS] token at the end of the image patch sequences, instead of at the beginning as in ViT, to enable the causal self-attention module to capture information from each image patch. 
% Our proposed methods demonstrate that through only \textit{supervised training}, a \textit{non-autoregressive decoder-only} architecture can surprisingly also be used as an image classifier.
% Moreover, MLLM
% We hope DoiT can bring fresh prospects for the component-level alignment of language and vision architectures. 
 



% Decoder-only Transformers, represented by LLaMa, have become the preferred choice for large language models (LLMs), for their contribution to the dramatic increase of linguistic capabilities. However, on the visual side, an encoder-only Transformer, such as ViT, are conventionally favored as the default selection. Can we alleviate this architectural gap? In this paper, we answer this question by introducing \textit{Decoder-only vision Transformer (DoiT)}. Our findings are a \textit{supervised trained non-autoregressive decoder-only} Transformer architecture can surprisingly also be used as an image classifier. By striving to align with the LLaMa decoder, we gradually adapt its components to our DoiT architecture. During our exploration, we propose to place the learnable class token at the end of the sequences of image patches, rather than at the head as in ViT, so that information of each patches of the image can be obtained through the causal self-attention module. DoiT offers possibilities and initial support for achieving component-level unification of language and visual architectures.


% 做出来就替换这一段：
% Decoder-only Transformers, represented by LLaMa, have become the preferred choice for large language models (LLMs), for their contribution to the dramatic increase of linguistic capabilities. However, on the visual side, an encoder-only Transformer, such as ViT, are conventionally favored as the default selection. Can we alleviate this architectural gap? In this paper, we answer this question by introducing \textit{Decoder-only vision Transformer (DoiT)}. Our findings are twofold: 1) a \textit{supervised trained non-autoregressive decoder-only} Transformer architecture can surprisingly also be used as an image classifier. 2) xxx. By striving to align with LLaMa decoder, we gradually adapt its components to our DoiT network. During our exploration, we propose two simple yet effective improvements: 1) we propose to place the learnable class token at the end of the sequences of image patches, rather than at the head as in ViT, so that information of each patches of the image can be obtained through the causal self-attention module. 2) xxx. DoiT offers possibilities and initial support for achieving component-level unification of language and visual architectures.

% DoiT set a new path to the unification of the architectural design of the language and vision backbones and provide technical support for the construction of decoder-only multi-modal LLMs. 



% 这一段模仿 DINO 写的，也不错：
% This paper investigates whether decoder-only architecture that serves as the favored choice for large language models (LLMs), can also accommodate visual Transformers through only \textit{supervised learning}. 
% We literally summarize our conclusions to two folds:
% Our conclusions are twofold: 
% 1) a \textit{supervised trained non-autoregressive decoder-only} Transformer architecture can surprisingly also be used as an image classifier. 
% 2) ...
% At the begining, we aim to align with the LLaMa decoder architecture, gradually adapting its components to the visual network. 
% During our exploration, we propose two simple yet effective improvements: 
% 1) we propose to place the learnable class token at the end of the sequences of image patches, rather than at the head as in ViT, so that information of each patches of the image can be obtained through the causal self-attention module.
% 2) ...
% Our proposed model are named as \textit{Decoder-only vision Transformer (DoiT)}. 
% Its decoder-only property offers the possibility of designing multimodal models of vision and LLMs with a unified design.
% DoiT set a new path to the unification of the architectural design of the language and vision backbones and provide technical support for the construction of decoder-only multi-modal LLMs. 


% With its decoder-only property, DoiT set a new path to the unification of the architectural design of the vision and language models.











% Decoder-only Transformers, represented by LLaMa, have become the preferred choice for large language models (LLMs). However, on the visual side, a Transformer encoder, such as ViT, are conventionally favored as the default selection. Due to this architectural gap, the network details of vision backbone and LLMs have not yet been fully harmonized. To bridge this gap, we construct a non-autoregressive decoder-only backbone similar to LLaMa with as few modification as possible. Specifically, we propose to place the learnable class token at the end of the sequences of image patches, rather than at the head as in ViT, so that information of each patches of the image can be obtained through the causal self-attention module. Surprisingly, through \textit{supervised training} only, this network can achieve comparable performance to the encoder-only ViT in ImageNet classification tasks, and we name it \textit{Decoder-only vision Transformer (DoiT)}. This discovery set a new path to the unification of the architectural components of the vision and language backbones and provide support for the construction of decoder-only multi-modal LLMs. 

% 以 LLaMa 为代表的 Decoder-only 的 Transformer成为了大语言模型的优选。
% 但是在其视觉层面，模型架构一般还是会默认选取 Transformer Encoder。
% 因为这个架构差异，视觉和语言模型的架构还没完全统一。
% 为了bridge the gap，我们构建了一个 non-autoregressive decoder-only backbone。
% 我们提出将可学习的 "类别标记 "放在图像片段序列的末尾，而不是像 ViT 那样放在头部，这样就可以通过 LLaMa 中的 causal self-attention 模块获取图像的全局信息。
% 惊讶的是，仅仅通过有监督训练，这样 Decoder-only 的视觉骨干模型可以在 ImageNet 图像分类任务中获得与 Encoder-only 的 ViT 架构十分相当的性能。
% 这一发现为统一视觉和语言基础模型的架构细节开辟了一条新路，并为构建大型 decoder-only 的多模态架构奠定了基础。





% In this paper, we demonstrate that a decoder-only architecture similar to LLaMa, through \textit{supervised training} only, can be used on a vision Transformer , and we name it \textit{Decoder-only vision Transformer (DoiT)}. We propose to place the learnable class token at the end of the sequences of image patches, rather than at the head as in ViT, so that information of each patches of the image can be obtained through the causal self-attention module. We empirically show that such decoder-only backbone can achieve comparable performance to the encoder-only ViT in ImageNet image classification tasks. This discovery set a new path to the unification of the architectural components of the vision and language backbones and provide support for the construction of decoder-only multi-modal LLMs. 




% 以 LLaMa 为代表的 Decoder-only 的 Transformer 架构助力了语言 Transformer 尺寸的放大和能力的大幅提升，成为了大语言模型的优选。
% 但是在其视觉层面，模型架构一般使用 Transformer Encoder。
% 在本文中，我们并不提出新的方法，而是证明了 LLaMa Decoder-only 架构，通过有监督训练，可以在尽可能不做任何修改的条件下用于视觉 Transformer 上面。
% 我们提出将可学习的 "类别标记 "放在图像片段序列的末尾，而不是像 ViT 那样放在头部，这样就可以通过 LLaMa 中的 causal self-attention 模块获取图像的全局信息。
% 我们实证性地展示出这样 Decoder-only 的视觉骨干模型可以在 ImageNet 图像分类任务中获得与 Encoder-only 的 ViT 架构十分相当的性能。
% 这一发现为统一视觉和语言基础模型的架构细节开辟了一条新路，并为构建大型 decoder-only 的多模态架构奠定了基础。














\end{abstract}
